Telco-DPR: A Hybrid Dataset for Evaluating Retrieval Models of 3GPP Technical Specifications

This paper proposes a Question-Answering (QA) system for the telecom domain using 3rd Generation Partnership Project (3GPP) technical documents. Alongside, a hybrid dataset, Telco-DPR, which consists of a curated 3GPP corpus in a hybrid format, combining text and tables, is presented. Additionally, the dataset includes a set of synthetic question/answer pairs designed to evaluate the retrieval performance of QA systems on this type of data. The retrieval models, including the sparse model, Best Matching 25 (BM25), as well as dense models, such as Dense Passage Retriever (DPR) and Dense Hierarchical Retrieval (DHR), are evaluated and compared using top-K accuracy and Mean Reciprocal Rank (MRR). The results show that DHR, a retriever model utilising hierarchical passage selection through fine-tuning at both the document and passage levels, outperforms traditional methods in retrieving relevant technical information, achieving a Top-10 accuracy of 86.2%. Additionally, the Retriever-Augmented Generation (RAG) technique, used in the proposed QA system, is evaluated to demonstrate the benefits of using the hybrid dataset and the DHR. The proposed QA system, using the developed RAG model and the Generative Pretrained Transformer (GPT)-4, achieves a 14% improvement in answer accuracy, when compared to a previous benchmark on the same dataset.

==> backup_files/01.Introduction.tex <==
\section{Introduction}
\label{sec:intro}

In the telecommunication (telecom) domain, multiple applications of \gls{genai} are envisioned for the upcoming \gls{6g} and legacy networks to boost the achievement and planning of all the requirements \cite{bariah2023large, maatouk2024largelanguagemodelstelecom, tarkoma2023ainativeinterconnectframeworkintegration, zhou2024large}. 
The major player in primary standardisation in wireless networks is the \gls{3gpp} in telecommunications \cite{3gpp_specifications}, which has been responsible for developing universal standards for \gls{3g}, \gls{4g}, and \gls{5g}. Understanding these protocols is crucial for engineers and researchers developing new devices and optimisation actions in compliance with the standards, ensuring seamless compatibility.

Current \gls{qa} systems heavily rely on \glspl{llm}. However, these \glspl{llm} are typically trained on a corpus of general knowledge extracted from the internet. In the case of a telecom corpus, which contains domain-specific knowledge, specialised jargon, and complex language, general \glspl{llm} are often inadequate for open-domain \gls{qa} systems, as they struggle to handle such intricate terminology effectively \cite{kandpal2023largelanguagemodelsstruggle}. 

To handle domain-specific \gls{qa}, several techniques are used in conjunction with \glspl{llm}. One such technique is domain-specific fine-tuning, which involves retraining a portion of the model's parameters to better adapt to specialised data \cite{roberts2020knowledgepackparameterslanguage}. However, this approach can be computationally expensive. A more lightweight alternative is the \gls{rag} method \cite{dai2019transformerxlattentivelanguagemodels}. \gls{rag} operates in two sequential steps: first, a retriever system identifies and retrieves passages that could assist in answering a question. These retrieved passages are then provided to a reader system—often a transformer-based model—which uses this context to interpret and extract the answer to the question.


Most retrieval techniques are designed primarily to handle unstructured text. However, in many fields, such as scientific literature and technical product documentation, information is often presented in a hybrid format that includes text, figures, and semi-structured tables. These tables and figures are typically interspersed with the text and are cross-referenced within the same document, providing essential supplementary or complementary semantic information\cite{chen2021openquestionansweringtables}. %This structure necessitates that QA systems perform multi-hop inference across images, tabular data, and unstructured text, as the evidence required to answer a question may be spread across these different input types, making evidence retrieval particularly challenging .

The objective is to develop a \gls{qa} system leveraging the advanced \gls{rag} technique specifically for \gls{3gpp} standards, taking into account the structured nature of the documents, which include both text and tables. 



%SELF-RAG: LEARNING TO RETRIEVE, GENERATE, AND CRITIQUE THROUGH SELF-REFLECTION->
% indiscriminately retrieving and incorporating a fixed number of retrieved passages, regardless of whether retrieval is necessary, or passages are relevant, diminishes LM versatility or can lead to unhelpful response generation.

%ADD PAPER CITATION: Tables to Latex:structure  and content extraction from scientific papers


The assessment of the retriever part was made by \cite{doringer2023synthetic},  a retriever-reader-based architecture was present and 
adapted to a corpus of Telecom documents. The assementment of the retriever part was made using a synthetic dataset from 3GPP documents, and it compared
the usage of a dense retriever using BERT to a BM25-based retriever on the
domain. Findings suggest the improvment increasing the Top-K retrieval
accuracy by 20 points for k = 10 when the embeddings are fine-tuning, compared to a general dense retriever. However, the dataset yield in this work is private.

In summary, the main contributions of this paper are:
\begin{itemize}
    \item The release of a publicly available dataset based on \gls{rag} standards, taking into account the structured organisations of the documents.
    \item An evaluation of the retriever's performance in \gls{qa} tasks using a telecommunications corpus.
\end{itemize}




%The paper is organized as follows: Following the introduction, Section II explores related work and introduces the proposed  methodology. Section III presents the experimental study, utilizing live network data to evaluate the dynamic approach of the proposed methodology, while comparing it to a fixed threshold approach. In Section IV, conclusions are drawn, and future work is outlined.

==> backup_files/02.RelatedWork.tex <==
\section{Related Work}

The study in \cite{huang2023largelanguagemodelsnetworking} introduces ChatNet, which leverages \glspl{llm} as orchestrators for external network tools used in network planning tasks. 
Notably, recent studies such as \citep{bariah2023large} have showcased promising outcomes for the \gls{nlp} tasks. In this research, a variety of \glspl{llm}, including \gls{bert}, \gls{roberta}, and \glspl{gpt}, were fine-tuned to Telecom domain languages for the classification of working groups within the \gls{3gpp} through technical specification analysis. 
Two notable studies in troubleshooting have been highlighted. The first one by \citep{alexander2022automated} focused on converting unstructured trouble reports into embeddings using various pre-trained language models to group similar trouble reports. The study found that the S-BERT sentence model outperformed other BERT-based language models. Another study \citep{i2021natural} aimed at automating the retrieval of solutions for troubleshooting reports in the telecommunications industry, which often involve complex textual data. This work utilized \gls{bert} to rank solutions for new troubleshooting reports using historical data, employing a multi-stage architecture with both retrieval and re-ranking stages.

Question-answering on long documents is a challenging real-world task that has attracted increasing attention in recent years.
In this domain, promising results have already been demonstrated for \gls{qa} applications. For instance, \cite{holm2021bidirectional} highlights the benefits of fine-tuning on a general-domain, and \cite{karim2023spec5gdataset5gcellular} illustrates the advantages for \gls{5g} protocol security-related text classification and summarization.


The TeleQnA dataset, as outlined in \citep{maatouk2023teleqna}, is primarily utilised as a benchmark for comparing language models about telecom-related knowledge. Originating from an extensive collection of telecom-specific documents, this dataset comprises multiple-choice questions structured with a question, answer choices, a correct answer, and an explanation. While the TeleQnA dataset primarily concentrates on evaluating language models in a zero-shot learning scenario, another dataset called SPEC5G \citep{karim2023spec5gdataset5gcellular} that have  \gls{4g}/\gls{5g} specifications and web sources, encompassing a wide array of materials such as method and framework documentation, pseudocode, high-level implementations, and parameters. However, all releases are contained within a single document, lacking indications of their respective start and end points.

%\cite{yilma2024telecomragtamingtelecomstandards}
%cite: THE CHRONICLES OF RAG: THE RETRIEVER, THE CHUNK AND THE GENERATOR
